Less is More! A slim architecture for optimal language translation

The softmax attention mechanism has emerged as a noteworthy development in the field of Artificial Intelligence research, building on the successes of Transformer-based architectures. However, their ever increasing sizes necessitate ever increasing computational memory, that limits their usage. We propose KgV, a sigmoid gating mechanism that, in conjunction with softmax attention, significantly boosts performance without increasing architecture size. To amend the size requirements, we leverage Tensor Chains to identify and prune the excess parameters. We find that such excess resides primarily within the embedding layer, and not in the output linear layer. To further improve embedding and significantly reduce parameters, we introduce H-SoftPOS, a hierarchical embedding layer which simultaneously enhances performance. Remarkably, on the WMT14 English-German validation set, our approach yields a threefold reduction in perplexity, surpassing the current state-of-the-art, while reducing parameter counts also by a factor of 3. When we further reduce the number of parameters up to sevenfold, we can still achieve a 21\% decrease in perplexity with respect to the baseline Transformer. To understand generalization capabilities, we conduct experiments on the 7 language pairs of the WMT17 dataset. Our method outperforms existing techniques in terms of test loss while simultaneously halving the number of parameters. Moreover, we observe a 70 times reduction in variance with respect to the prior state-of-the-art. In conclusion, our proposed method yields significant improvements in performance and much lower memory cost. We call the resulting architecture Anthe.

==> sections/old_text.tex <==


\begin{table}[h]
\centering
\begin{tabular}{lcccc}
\toprule
& & CS/EN & DE/EN & FI/EN \\
dataset size & & 1.6G & 8.1G & 3.9G \\
& params & val PPL & val PPL & val PPL  \\
\midrule
Anthe  & 30M & $\textbf{4.2196} \pm \textbf{0.0129}$ &  $\textbf{3.8554} \pm \textbf{0.0117} $ & $\textbf{4.1666} \pm \textbf{0.0092}$ \\
Anthe$_{no TT}$  & 68M & $4.6400 \pm 0.0350$ &  $5.1376 \pm 0.0429$ & $5.4544 \pm 0.0182$ \\
Transformer & 60M & $5.1493 \pm 0.0384$ & $6.1099 \pm 0.5296$ & $5.8418 \pm 0.0801$ \\  
\midrule
\bottomrule \\
\end{tabular}

\vspace{.5cm}

\begin{tabular}{lrcccc}
\toprule
 & & LV/EN & RU/EN & TR/EN & ZH/EN\\
 & & 4.3G & 9G & 306M & 9G \\
& params & val PPL & val PPL & val PPL & val PPL  \\
\midrule
Anthe  & 30M & $\textbf{8.1622} \pm \textbf{0.1882}$ & $\textbf{4.1564} \pm \textbf{0.0026}$ & $\textbf{3.9664} \pm \textbf{0.0046}$ & $\textbf{7.1757} \pm \textbf{0.0460}$ \\
Anthe$_{no TT}$  & 68M & $\textbf{8.1644} \pm \textbf{0.0918}$ & $6.6792 \pm 0.1127$ & $\textbf{3.9627} \pm \textbf{0.0158}$ & $11.0325  \pm 0.3977$ \\
Transformer & 60M & $10.0284 \pm 0.8826$ & $8.3311 \pm 0.1627$ & $5.1725 \pm 0.0210$  &  $17.9119 \pm 0.2986$\\ 
\midrule
\bottomrule \\
\end{tabular}
\caption{\textbf{Different Datasets.} WMT17, The FiLMformer outperforms. TR/EN is the smallest dataset, so it might not have enough data to draw a conclusion.}
\label{tab:vallangs}
\end{table}

\section{Plan}


\section{Skip connections counteract self-attention}

Possibly fully prove section 3.1 of \citep{dong2021attention}


\subsubsection{More Skip Connections}

We introduce two types of skip connections, one between encoder and decoder, and the other within.  
We call \textit{stairs} the horizontal connections in Fig.~\ref{fig:architecture_layout}. Instead of connecting the last decoder block to all the encoder blocks, we pass each encoder block representation to the decoder block that is at the same depth. The second type is vertical, within either the encoder or within the decoder, and we call them \textit{2-skip} connections. We take the output of every block, after the FiLM fusion (see below), we skip two blocks, and we add it to the output of the second block, before passing it through a ReLU activation, and use it as input to the following block. \red{Vertical skip connections don't seem to improve performance now. Send experiments with softPOS and MPO without the 2 skips.}



\subsubsection{FiLM Modulation}

Transformers typically deal with what can be understood as modality fusion, where the encoder takes care of one sensory modality (e.g. the language to translate from) and the decoder takes care of the another (e.g. the language to translate to). However, the Transformer passes only the last representation of the decoder to the encoder. This is in contrast with what has been observed in the modality fusion literature \cite{de2017modulating, ronneberger2015u, perez2018film, hosseini2022end}, that suggests that different modalities benefit from specialized processing pipelines, that need to be able to influence each other at different steps in the processing hierarchy. This experimental observation is in line with what has been discovered theoretically \citep{dong2021attention}: skip connections and
MLPs stop the rank degeneration produced by the attention mechanism, and increasing the path length diversity is therefore beneficial.

In addition to these skip connections, we augment the connectivity between encoder and decoder through FiLM connections~\citep{perez2018film}. If $x_l$ is the vector representation of a sensor modality, and $y_l$ the vector representation of another sensor modality, FiLM is described by the following linear modulation
\begin{align}
    x_l = F iLM(x_{l-1}, y_{l-1}) = \gamma(y_{l-1}) x_{l-1} + \beta(y_{l-1})
\end{align}
\noindent where $\gamma, \beta$ don't need to be linear functions. In our case, both are represented by 1D convolutions, with $d_{model}$ number of filters, and causal kernels of size 3. When we use dilation, we increment it with depth $l$ as $2^l$ to increase the effective kernel size. Moreover we use 2 FiLMs in opposite directions at each layer, so we also have two  $\gamma$ and two  $\beta$ convolutions. Therefore in one direction $x_{l-1}, y_{l-1}$ are the outputs of the encoder and the decoder respectively, while on the other directions they are the outputs of the decoder and the encoder respectively. \red{The two way FiLM might be breaking the causality of the decoder, repeat the experiments with one way FiLMs.}


